Multiplicity-free representations of the symmetric group

We determine all the multiplicity-free representations of the symmetric group. This project is motivated by a combinatorial problem involving systems of set-partitions with a specific pattern of intersection.

==> tables <==
For three families of groups ( $S_2 \wr A_k$, $(S_2^k \cap
A_{2k})\rtimes S_k$ and $S_1 \times (S_2 \wr S_k)$ ) the rank is too
complicated to be included in the table.

\begin{table}[h]
\begin{center}
\begin{tabular}{l ccc}
Group & $n$ & index & rank\\
$A(n)$ & $n$ & $2$ & 2 \\
$S(n)$ & $n$ & $1$ & 1 \\
$AGL(1,5) \cap A_5$ & 5 & 12 & 4\\
$AGL(1,5)$ & 5 & 6 & 2 \\
$PSL(2,5)$ & 6 & 12 & 4 \\
$PGL(2,5)$ & 6 & 6 & 2 \\
$AGL(1,7)$ & 7 & 120 & 7 \\
$PSL(3,2)$ & 7 & 30 & 4 \\
$A\Gamma L(1,8)$ & 8 & 240 & 8 \\
$PGL(2,7)$ & 8 & 120 & 5 \\
$AGL(3,2)$ & 8 & 30 & 4 \\
$AGL(2,3)$ & 9 & 840 & 9 \\
$P\Gamma L(2,8)$ & 9 & 240 & 5 \\
$\aut(PSL(2,9))$ & 10 & 2520 & 10 \\
$M_{11}$ & 11 & 5040 & 10 \\
$M_{11}$ & 12 & 60480 & 26 \\
$M_{12}$ & 12 & 5040 & 8 \\
\end{tabular}
\caption{Multiplicity-free transitive primitive groups. \label{table:transitive}}
\end{center}
\end{table}

\renewcommand{\arraystretch}{1.25} 
\begin{table}
\begin{center}
\begin{tabular}{lccc}
Group & $n$ & index & rank\\
$S_\ell \wr S_2$ & $2\ell$ & $\frac{1}{2}{2\ell \choose \ell}$  & ${\lfloor \ell/2 \rfloor }+1$ \\
$(S_\ell\wr S_2)\cap A_{2\ell}$, $\ell \geq 3$ & $2\ell$ & ${2\ell \choose \ell}$ &  $2(\lfloor \ell/2 \rfloor +1 )$ \\
$((S_\ell \times S_\ell) \cap A_{2\ell})\rtimes S_2$, $\ell \geq 3$ &$2\ell$ &${2\ell \choose \ell}$ & $2(\lfloor \ell/2 \rfloor +1 )$ \\
$A_\ell \wr S_2$, $\ell \geq 3$  & $2\ell$ & $2{2\ell \choose \ell}$ & $2(\lfloor \ell/2 \rfloor +1 ) +2$\\
$AGL(1,5) \wr S_2$ & 10 & 4536 & 16 \\
$PGL(2,5) \wr S_2$ & 12 &  16632 & 13 \\

$S_2\wr S_k$  & $2k$ & $\frac{(2k)!}{2^k k!}$ & $p(k)$ \\
$(S_2\wr S_k) \cap A_{2k}$, $k$ odd & $2k$ & $\frac{(2k)!}{2^{k-1} k!}$ & $2p(k)$ \\ 

$S_2 \wr A_k$ & $2k$ & $\frac{(2k)!}{2^{k-1} k!}$ &  \\
\ ($k \in (3,4,7,8,11,12,16,20,24)$) & & & \\

$(S_2^k \cap A_{2k}) \rtimes S_k$ & $2k$ & $\frac{(2k)!}{2^{k-1} k!}$ &  \\
\ ($k\in\{2,\! 4,\!5,\!6,\!8,\!9,\!12,\!13,\!16,\!17,\!20,\!24,\!28,\!32\}$)& & & \\

$S_3 \wr S_3$ & 9 & 280 & 5 \\
$(S_3 \wr S_3) \cap A_9$ & 9 & 560  & 10 \\
$((S_3)^3 \cap A_9) \rtimes S_3$ & 9 & 560  & 9 \\
$S_3 \wr S_4$ & 12 & 15400  & 12 \\
$(S_3 \wr S_4) \cap A_{12}$ & 12 & 30800 & 24 \\
$S_4 \wr S_3$ & 12 & 5775 & 9 \\
$(S_4 \wr S_3) \cap A_{12}$& 12 & 11550 & 18\\
$((S_4)^3 \cap A_{12}) \rtimes S_3$& 12 & 11550 & 16 \\
$SD_4$ & 12 & 23100& 18 \\
$RD_4$ & 12 & 46200 & 33\\
$S_5 \wr S_3$ & 15 & 126126 & 13 \\
$(S_5 \wr S_3)\cap A_{15}$ & 15 &252252 & 26\\
$((S_5)^3 \cap A_{15}) \rtimes S_3$ & 15 & 252252 & 25\\
$SD_5$ & 15 &504504 & 24\\
$A_5 \wr S_3$ & 15 & 1009008 & 46 \\
\end{tabular}
\caption{Multiplicity-free transitive imprimitive groups\label{table:imprimitive}
}
\end{center}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{lccc}
Group & $n$ & index & rank\\
$S_1 \times AGL(1,5)$ & $6$ & 36 & 5 \\
$S_1 \times PSL(2,5)$  & 7 & 84 & 8\\
$S_1 \times PGL(2,5)$  & 7 & 42 & 4 \\
$S_1 \times PSL(3,2)$ &  8 & 240 & 10\\
$S_1 \times PGL(2,7)$ &  9 & 1080 & 12\\
$S_1 \times AGL(3,2)$ &  9 & 270 & 8 \\
$S_1 \times P\Gamma L(2,8)$  & 10 & 2400 & 13 \\
$S_1 \times M_{12}$ &  13& 65520 &18 \\
$S_2 \times PSL(2,5))$  & 8 & 336 & 11\\
$S_2 \times PSL(3,2)$  & 9 & 1080 & 14 \\
$S_2 \times AGL(3,2)$  & 10 & 1350 & 11\\
$S_2 \times P\Gamma L(2,8)$ & 11 & 13200 & 20\\
$S_2 \times M_{12}$ & 14 & 458640 & 28 \\
$S_3 \times AGL(3,2)$ & 11 & 4950 & 13\\
$A_3 \times AGL(3,2)$ & 11 & 9900 & 26 \\
$S_3 \times P\Gamma L(2,8)$ & 12 & 52800 & 26 \\
$S_3 \times M_{12}$ & 15 & 2293200 & 37 \\
$S_4 \times P\Gamma L(2,8)$ & 13& 171600 & 30 \\
$S_4 \times M_{12}$ & 16 & 9172800 & 44 \\
$S_5 \times M_{12}$ & 17 & 31187520 & 48 \\
\end{tabular}
\caption{Multiplicity-free intransitive groups\label{table:intrans}}
\end{center}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{llccc}
Group & & $n$ & index & rank\\
$S_k \times S_{n-k}$ & $(2k \leq n)$ & $n$ & ${n \choose k}$ & $k+1$ \\
$(S_k \times S_{n-k})\cap A_{n}$ & $(2k\leq n$, $(k,n)\neq (2,4))$& $n$ & $2{n \choose k}$ & $2k+2$ \\
$A_k \times S_{n-k}$ & $(2k \leq n$, $k \neq 2)$ & $n$ & $2{n \choose k}$ &  $k+3$\\
$S_k \times A_{n-k}$ & $(2k \leq n$, $k \neq n-2)$ & $n$ & $2{n \choose k}$ &  $k+3$\\
$A_k \times A_{n-k}$ & $(k\geq 3$, $2k \leq n-2)$ & $n$ & $4{n \choose k}$ &  $2k+6$\\

$S_k \times AGL(1,5)$ & $(k\geq 2)$ & $k+5$ & $\frac{(k+5)!}{20 (k!)}$ & $k+5$ \\
$A_k \times AGL(1,5)$ & $(k\geq 4)$ & $k+5$ & $\frac{(k+5)!}{10 (k!)}$ & $k+13$ \\
$(S_k \times (AGL(1,5)) \cap A_{k+5}$ &$(k\geq 5)$ & $k+5$ & $\frac{(k+5)!}{10 (k!)}$ & $2k+10$ \\

$S_k\times PGL(2,5) $ & $(k\geq 2)$ & $k+6$ & $\frac{(k+6)!}{120 (k!)}$ & $k+4$ \\
$A_k \times PGL(2,5) $ & $(k\geq 3)$ & $k+6$ & $\frac{(k+6)!}{60 (k!)}$ & $k+10$ \\
$(S_k \times (PGL(2,5)) \cap A_{k+6}$& $(k\geq 2)$ & $k+6$ & $\frac{(k+6)!}{60 (k!)}$ & $2k+8$ \\

$S_k\times P\Gamma L(2,8) $ & $(k\geq 5)$ & $k+9$ & $\frac{240 (k+9)!}{9!k!}$ & \small{$27\!+\!\min\{ k, \lfloor \frac{k+9}{2} \rfloor\}$}\\

$S_1 \times (S_k \wr S_2)$ & &$2k+1$ & $\frac{(2k+1)!}{2(k!)^2}$ & $3\lfloor \frac{k}{2}\rfloor$\\
$(S_1\times((S_k \wr S_2))\cap A_{2k+1})$& $(k \geq 3)$&$2k+1$ &$\frac{(2k+1)!}{(k!)^2}$&$6\lfloor \frac{k}{2}\rfloor$\\
$(S_1\times ((S_k^2 \cap A_{2k})\rtimes S_2)$ & $(k \geq 3)$ &$2k+1$ &$\frac{(2k+1)!}{(k!)^2}$&$6\lfloor \frac{k}{2}\rfloor$\\

$S_1 \times (S_2 \wr S_k)$&& $2k+1$ & $\frac{(2k+1)!}{2^k k!}$ & \\
\end{tabular}
\caption{Multiplicity-free intransitive groups, continued \label{table:intrans2}}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1} 

